Identifying Distributional Perspective Differences from Colingual Groups

Perspective differences exist among different cultures or languages. A lack of mutual understanding among different groups about their perspectives on specific values or events may lead to uninformed decisions or biased opinions. Automatically understanding the group perspectives can provide essential background for many downstream applications of natural language processing techniques. In this paper, we study colingual groups and use language corpora as a proxy to identify their distributional perspectives. We present a novel computational approach to learn shared understandings, and benchmark our method by building culturally-aware models for the English, Chinese, and Japanese languages. On a held out set of diverse topics including marriage, corruption, democracy, our model achieves high correlation with human judgements regarding intra-group values and inter-group differences.

==> intro_old.tex <==
\section{Introduction}
\label{sec:intro}
%Culture is a hypernym  which includes the behavior and norms found in human societies, as well as the beliefs, knowledge, arts, laws, customs, capabilities and habits of the individuals in these groups\footnote{https://en.wikipedia.org/wiki/Culture}.~\violets{do we need this sentence?} %The relationship between language and culture is deeply rooted,
%\footnote{https://www.tefl.net/elt/articles/teacher-technique/language-culture/}
Stance Detection \cite{mohammad2016semeval,bar2017stance} represents a well established task in natural language processing and is often described by having two inputs: (1) a topic and (2) a statement made by an author. Given these two inputs, the aim is to find out whether the author is in favor of or against the topic. Most work in stance detection has been limited to mono-lingual settings, in particular for English, but less attention has been paid to other languages represented by a particular culture. 
Languages and cultures have radical correlations as individuals communicate with each other by language, which carries the aspects of their culture: their prior beliefs, attitudes and values \cite{khaslavsky1998integrating}. 
Hence, understanding the differences in stances among various cultures can play a vital role in understanding expectations of people from different national and cultural backgrounds. 
%For example, a  model enables better downstream applications such as more pragmatic machine translation or cultural-aware sentiment analysis. %It can also be utilized by transnational organizations, such as multi-national enterprises, for more efficient delivery of information across various regions. %Therefore, understanding cross cultural similarities and differences lies at the crux of cross-lingual natural language understanding. 

\begin{table}[t!]
\setlength{\belowcaptionskip}{-0.7cm}
\small
\begin{tabular}{|p{1.15cm}|p{5.6cm}|}
\hline
English                                                                & \begin{tabular}[c]{@{}l@{}}\textit{In contrast, unsafe abortions (those }\\\textit{performed by unskilled individuals,with }\\\textit{hazardous equipment, or in unsanitary }\\\textit{facilities) cause 47,000 deaths and 5 }\\\textit{million hospital admissions each year.}\end{tabular}                                                                                        \\ \hline\hline
 Chinese                                                                 &\begin{CJK}{UTF8}{gkai} \begin{tabular}[c]{@{}l@{}}据不完全统计中国由于以往进行的一孩\\政策（每对夫妇只容许有一个子女），\\每年人工流产至少1300万例， 位居世界\\第一。… \textit{\color{red}{人们对堕胎的反对较受基督教}}\\\textit{\color{red}{教义影响的西方国家低}}，在中国计划生育\\政策的背景下，很多人采取自愿堕胎，部\\分是婴儿的性别因素（重男轻女）也有人\\被计生部门实行强制堕胎（如残疾等）。
 \end{tabular}   \end{CJK}                                                               \\ \hline
\begin{tabular}[c]{@{}l@{}}Translated\\ English\\ Version\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textit{Due to the one-child policy in China (each}\\ \textit{couple only allowed one child), China has} \\\textit{at least13 million abortions per year, ranking }\\\textit{first in the world,… \color{red}Opposition to abortion }\\\textit{\color{red}{is lower than in western countries influenced}}\\ \textit{\color{red}{by Christianity}. \color{black}{In the context of China's } }\\\textit{family planning policy, many people have}\\ \textit{abortions of their own free will, partly}\\ \textit{because of the  gender of the baby (prefer}\\\textit{ence  for sons) and partly because of forced}\\ \textit{ abortions by family planning authorities} \\\textit{ (disability, etc.).}\end{tabular} \\ \hline
\end{tabular}
\caption{Wikipedia excerpts from English and Chinese Wikipedia page of Abortion exemplifying opposite stance on the same topic from two different cultures. Note that either selected sentence is unique in its own languages and non-existent in the page of the other language.}
\label{table:example1}

\end{table}\violets{Similarly, we need to change these examples (in Table~\ref{table:example1}) to some topics that are less controversial within a group.}
  
%Humans can easily discern and identify cultural differences through commonsense or world knowledge. 
%commonsense knowledge influences human experience, encompassing knowledge about the spatial, physical, social, temporal and psychological aspects of day to day life.
Even though beliefs/values are tacitly shared within a culture, cultural knowledge is usually concealed in written texts. While there has been an increasing interest in  Cross-Lingual Stance Detection \cite{mohtarami2019contrastive}, current works are mostly limited to leveraging resources from a source language to train a model in a target language. They do not explicitly model the cultural reflection in the source and the target languages that leads to opposing stances. Recently, \newcite{lin-etal-2018-mining} present a distributional approach to compute cross-cultural differences (or similarities) between two aligned terms. However, the approach focuses on word-level (named entities in particular) semantics, which is hard to be generalized to other forms.
% in teaching machines commonsense knowledge \cite{comet,sap2019atomic,huang2019cosmos,sap2019socialiqa}, little light has been shed on systematic approaches to represent knowledge about cultural differences.


We contribute models that identify opposing stances from different cultures by recognizing \textit{claims} that are culturally disagreed upon. Cultural models shape the social identities of those that ascribe to them~\cite{Geertz}, and help members of that culture to interpret the world in a shared manner. Cultural models can inform a number of different categories of daily life, including which foods are edible, how to form social ties, and which values are agreeable. In this work, we use natural language claims to represent cultural models. Claims such as \textit{``Abortion should be made illegal''} is a stance against abortion that reflects the cultural belief of a certain community.
% This claim is viewed very differently by \textbf{Tuhin: I am not sure if we should add this still \textit{English-speaking}} and Chinese-speaking cultures.
Despite a lack of consensus within English-speaking cultures, support for this statement is much greater in English-speaking cultures than in Chinese-speaking ones where there has been a ``wide awareness and acceptance of abortion [...] since antiquity''~\cite{10.2307/189264}. Table \ref{table:example1} shows an example on this topic, where the Chinese and English Wikipedia pages reflect the underlying differences in stance between two cultures. %With the proper world knowledge, we know that abortion is commonly accepted in China, but it is not the case in the western world which is affected by the Christian doctrine. 
% Learning cultural models through text will enable researchers to understand differences between cultures with fineness. This is especially necessary with ad-hoc cultures emerging from interactions in daily life such as internet cultures.

The two east-asian countries, China and Japan, share similar cultures and ideology. A Wikipedia page named \textit{Chinese influence on Japanese culture}\footnote{https://en.wikipedia.org/wiki/Chinese\_influence\_on\_Japanese\_culture} states how older elements of the Japanese culture such as Taoism, Buddhism, astronomy and language, have been influenced by China. Wikipedia also tells us that in the modern times Japan is known to have one of the most uncorrupted government, while China suffers corruption-related issues. \yufei{Somewhat lengthy as we have two motivated examples, but I wrote my observations anyways}

Considering the fact that culture is intrinsic to language, we take different languages to represent different cultures. We leverage Wikipedia to learn cultural models through text. Wikipedia has 301 languages, presents a diverse array of topics, and hence can serve as an ideal source to understand difference in stances from respective cultures. 
%The content we find in multilingual Wikipedia pages is consistent with our commonsense knowledge. 
Despite Wikipedia's overall goal of objectivity, it embeds latent cultural bias. 

% In light of these observations, we propose a computational approach for understanding cultural difference leveraging multi-lingual Wikipedia. 
We summarize our contributions as follows:
\begin{itemize}
    \item  We propose Cultural Stance Difference Identifier (CSDI), a model that automatically learns opposing stances between respective cultures based on Wikipedia articles. Towards this, we develop a novel procedure for algorithmically generating negative samples (introduced in \ref{subsec:dataset creation}) based on Wikipedia.
    \item  We design an evaluation framework to systematically study the efficiency of the proposed approach by testing our models on self-labeled opinionated claims ranging through diverse topics including \textit{Food, Cuisine, Savings, Festivals, Marriage, Corruption, Terrorism, Democracy} and \textit{Privacy}.
    
    %\textit{\violets{fill in. no need to mention reddit yet.}}.%from the popular social media \textit{Reddit}.
    \item Comprehensive quantitative and qualitative studies in English, Chinese and Japanese show that our model outperforms multiple well-crafted baselines and achieves strong correlation with human judgements.\footnote{Our dataset and code will be released to the  community upon the paper acceptance.} %Qualitative results show our best model obtains strong correlation with human judgements and outperforms multiple well crafted baselines. 
\end{itemize}




% \cite{}
% \ref{table:example1} shows excerpts from Wikp
% \yfcomment{please include in the intro: 1) Although articles in Wikipedia are relatively objective, they are still somewhat biased, and hence we can utilize the uniqueness in each language versions. 2) Explain why the more-objective Wikipedia is better than online discussion forums like Reddit, where people express their subjective opinions. (First there is no such an open forum like Reddit in China, and second we expect opposite opinions during the discussion, and they mutually set off with each other. The model ends up feeling mixed towards most sentences.) Thanks! }\\
% \yfcomment{
% Or discuss it somewhere else, if intro is not the best place for those questions. 
%  }

